Multimodal perception for dexterous manipulation

Humans usually perceive the world in a multimodal way that vision, touch, sound are utilised to understand surroundings from various dimensions. These senses are combined together to achieve a synergistic effect where the learning is more effectively than using each sense separately. For robotics, vision and touch are two key senses for the dexterous manipulation. Vision usually gives us apparent features like shape, color, and the touch provides local information such as friction, texture, etc. Due to the complementary properties between visual and tactile senses, it is desirable for us to combine vision and touch for a synergistic perception and manipulation. Many researches have been investigated about multimodal perception such as cross-modal learning, 3D reconstruction, multimodal translation with vision and touch. Specifically, we propose a cross-modal sensory data generation framework for the translation between vision and touch, which is able to generate realistic pseudo data. By using this cross-modal translation method, it is desirable for us to make up inaccessible data, helping us to learn the object's properties from different views. Recently, the attention mechanism becomes a popular method either in visual perception or in tactile perception. We propose a spatio-temporal attention model for tactile texture recognition, which takes both spatial features and time dimension into consideration. Our proposed method not only pays attention to the salient features in each spatial feature, but also models the temporal correlation in the through the time. The obvious improvement proves the efficiency of our selective attention mechanism. The spatio-temporal attention method has potential in many applications such as grasping, recognition, and multimodal perception.

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}

  \section*{Sir Stanley Davidson (1894--1981)}

  One or more blank lines denote the end of a paragraph.  The ends of\index{index}
  words and sentences are marked by spaces. It doesn't matter how many
  spaces you type; one is as good as 100.  The end of a line counts as
  a space.

\end{biography}


==> chapter2.tex <==
\cleardoublepage

\begin{frontmatter}
\chapter{Chapter Title\footnote{This is chapter footnote}}\label{chap2}
\subchapter{Chapter Subtitle}

\begin{aug}
\author[addressrefs={ad1,ad2}]%
  {\fnm{Firstname}   \snm{Surname}}%
  %{\fnm{Firstname}   \snm{Surname}\footnote{This is author footnote}}%
\author[addressrefs={ad2}]%
 {\fnm{Firstname} \snm{Surname}}%
\address[id=ad1]%
  {Short Address}%
\address[id=ad2]%
  {Long Address}%
\end{aug}


% \minitoc

%
\begin{chapterpoints}%[Chapter Points]
\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
\end{chapterpoints}

\begin{dispquote}

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
  
  \source{Name}

\end{dispquote}

\end{frontmatter}


\section{Section title}\label{sec2.1}


==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}
  \name{Greg N. Gregoriou} is Professor of Finance in the School of
  Business and Economics at State University of New York at
  Plattsburgh. He obtained his Ph.D. (finance) from the University of
  Quebec at Montreal and is hedge-fund editor for the peer-reviewed
  scientific journal Derivatives Use, Trading and Regulation and
  editorial board member for the Journal of Wealth Management, and the
  Journal of Risk and Financial Institutions. He has written more than
  50 articles on hedge funds and managed futures in various U.S. and
  U.K. peer-reviewed publications, including (among others) the
  Journal of Portfolio Management, Journal of Derivatives Accounting,
  Journal of Futures Markets, European Journal of Operational
  Research, Annals of Operations Research, European Journal of
  Finance, and Journal of Asset Management. He has edited 18 books for
  Elsevier, Wiley, Palgrave-MacMillan, and Risk and has coauthored one
  book for Wiley.

  \name{Donald F. Dansereau} Department of Psychology, Texas Christian
  University, Fort worth, Texas

  \name{Ruth Garner} Department of Educational Psychology, Texas A \&
  M University, College Station, Texas
\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}

% Text ...


==> preface.tex <==
\cleardoublepage
\begin{frontmatter}
\chapter*{Preface}%
%\addcontentsline{toc}{schapter}{Preface}
\end{frontmatter}


 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

\source%
{%
  \author{Name}\\%
  % \address{Location}\\%
  % \date{Month Year}%
}


==> tableofcontents.tex <==
%% Table of Contents %%
\begin{frontmatter}
\chapter*{Contents}
\end{frontmatter}

\tableofcontents


==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  \begin{titlepagerule}
    \title{Book title}
    %\subtitle{Book Subtitle}
    %\volume{2}
  \end{titlepagerule}

  \edition{2nd edition}

%  \editedby{Edited by}

  \author{Author Firstname  Surname}
  \address{Author Address\\Department of Chemistry\\University of Florida}

  \author{Author Firstname  Surname}
  \address{Author Address}
\end{titlepage}

